Free-fermion descriptions of parafermion chains and string-net models

Topological phases of matter remain a focus of interest due to their unique properties -- fractionalisation, ground state degeneracy, and exotic excitations. While some of these properties can occur in systems of free fermions, their emergence is generally associated with interactions between particles. Here we quantify the role of interactions in general classes of topological states of matter in all spatial dimensions, including parafermion chains and string-net models. Using the interaction distance [Nat. Commun. 8, 14926 (2017)], we measure the distinguishability of states of these models from those of free fermions. We find that certain topological states can be exactly described by free fermions, while others saturate the maximum possible interaction distance. Our work opens the door to understanding the complexity of topological models and to applying new types of fermionisation procedures to describe their low-energy physics.

==> preamble.tex <==


% Command to conditionally typeset a bibliography.
\makeatletter
\newcommand\journal{\@journal}
\makeatother

\usepackage{pdftexcmds}


\makeatletter
\ifdefined\@journal

\ifnum\pdf@strcmp{\journal}{prl}=0 %
  \renewcommand{\section}[1]{\@startsection{section}{1}{\z@}%
                             {-3.25ex\@plus -1ex \@minus -.2ex}%
                             {-1.5ex \@plus -.2ex}% Formerly 1.5ex \@plus .2ex
                             {\indent\normalfont\normalsize\bfseries\itshape}{#1:--}}
\else
\fi
\fi

\makeatother

\usepackage{dcolumn}{}
\usepackage{bm}
\usepackage{amsfonts,amssymb,amsmath} 

\usepackage[dvipsnames]{xcolor}

\usepackage{tikz}

\usepackage{epstopdf}
\usepackage{mathbbol}

\usepackage{amsthm}


\usepackage{breakcites}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
%\newcommand{\theoremautorefname}{Theorem}

\theoremstyle{definition}
\newtheorem*{remark}{Remark}

\theoremstyle{remark}

\newcommand{\join}{\lor}
\newcommand{\meet}{\land}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bq}{\begin{eqnarray}}
\newcommand{\eq}{\end{eqnarray}}
\newcommand{\Sp}{\,\,\,\,\,\,}
\newcommand{\no}{\nonumber\\}
\newcommand{\lan}{\langle}
\newcommand{\ran}{\rangle}
\newcommand{\rf}[1]{(\ref{#1})}
\newcommand{\SIGMA}{\mbox{\boldmath${\sigma}$}}
\newcommand{\ALPHA}{\mbox{\boldmath${\alpha}$}}
\newcommand{\PSI}{\mbox{\boldmath${\psi}$}}
\newcommand{\PPSI}{\mbox{\boldmath${\Psi}$}}
\newcommand{\MU}{\mbox{\boldmath${\mu}$}}
\newcommand{\1}{1\!\!1}
\newcommand{\SSIGMA}{\mbox{\boldmath${\Sigma}$}}
\newcommand{\p}{{\bf p}} 
\newcommand{\rr}{{\bf r}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\ket}[1]{\left |#1 \right\rangle}
\newcommand{\bra}[1]{\left \langle #1 \right |}
\newcommand{\braket}[2]{\left \langle #1 \right| \left.#2\right\rangle}
\newcommand{\ketbra}[2]{\left| #1 \rangle \langle #2 \right|}
\newcommand{\jj}{{\boldsymbol{j}}}
\newcommand{\ii}{{\boldsymbol{i}}}
\newcommand{\sv}{\boldsymbol{s}}
\newcommand{\pp}{\boldsymbol{p}}
\newcommand{\zz}{\boldsymbol{z}}
\newcommand{\ep}{\boldsymbol{\epsilon}}
\newcommand{\cc}{\boldsymbol{c}}
\newcommand{\chris}[1]{{\textcolor{blue}{{#1}}}}
\newcommand{\kon}[1]{\textcolor{red}{#1}}
\newcommand{\ashk}[1]{\textcolor{OliveGreen}{#1}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}


\usepackage{wasysym}
\usepackage{soul}
\usepackage{tikz}

\usepackage{verbatim}

\usetikzlibrary{positioning,shapes.misc,calc,decorations.markings}
%########################################################
\tikzset{->-/.style={decoration={
      markings,
      mark=at position #1 with {\arrow{latex}}},postaction={decorate}}}
%########################################################
\tikzset{-<-/.style={decoration={
      markings,
      mark=at position #1 with {\arrow{latex reversed}}},postaction={decorate}}}
%########################################################
%########################################################
\usetikzlibrary{shapes.geometric}

\usepackage{amsfonts,amssymb,amsmath} 


\usepackage{float}
\usepackage[caption = false]{subfig}
\usepackage{graphicx}



